Combining Differential Privacy and Byzantine Resilience in Distributed SGD

Privacy and Byzantine resilience (BR) are two crucial requirements of modern-day distributed machine learning. The two concepts have been extensively studied individually but the question of how to combine them effectively remains unanswered. This paper contributes to addressing this question by studying the extent to which the distributed SGD algorithm, in the standard parameter-server architecture, can learn an accurate model despite (a) a fraction of the workers being malicious (Byzantine), and (b) the other fraction, whilst being honest, providing noisy information to the server to ensure differential privacy (DP). We first observe that the integration of standard practices in DP and BR is not straightforward. In fact, we show that many existing results on the convergence of distributed SGD under Byzantine faults, especially those relying on $(\alpha,f)$-Byzantine resilience, are rendered invalid when honest workers enforce DP. To circumvent this shortcoming, we revisit the theory of $(\alpha,f)$-BR to obtain an approximate convergence guarantee. Our analysis provides key insights on how to improve this guarantee through hyperparameter optimization. Essentially, our theoretical and empirical results show that (1) an imprudent combination of standard approaches to DP and BR might be fruitless, but (2) by carefully re-tuning the learning algorithm, we can obtain reasonable learning accuracy while simultaneously guaranteeing DP and BR.

==> rebuttal.tex <==
\section*{Rebuttal}
\subsection*{Reviewer 1}
We thank the reviewer for the feedback and provide our answers to their comments below.\\

\textbf{Answer to Q1:} Note that in our case, the server is not trusted, which is the main reason why our problem is challenging from a robust estimation perspective. We clarify this statement below by comparing the trusted server and non-trusted server settings.\

- If the server were trusted, it would have direct access to the workers' data and would only apply confidentiality when computing the robust statistic. In this case, as the reviewer points out, Byzantine resilience and robust estimation share some similarities. However, note that while the two problems seem close, in general, optimizing a non-convex function from corrupted gradients is more difficult than simply estimating the mean of a distribution from corrupted data samples.  

- In our context, the server is not trusted but rather honest-but-curious (see the threat model in Section 2). Therefore, the privacy mechanism is applied at the worker level before sending the gradients to the server for computing the robust statistic. In this case, the references provided by the reviewer are no longer applicable. The honest-but-curious assumption indeed makes the computation of robust statistics much more challenging, especially in non-convex settings where workers only send gradients.

\textbf{Answer to Q3:} We agree with the reviewer on this point. The function $b \mapsto \ln(b) (C + 1/b)^2$ need not be decreasing on $[1,m]$, especially when $C$ is not sufficiently small. However, by analyzing the variation of the function, we can see  that it is indeed decreasing on $(1,m]$ as soon as $C < \frac{2\ln{m} - 1}{m}$, which is equal to $3.5 \times 10^{-4}$ in our experiments ($m = 60,000$ for MNIST and Fashion-MNIST). In our paper, $C = \frac{1}{m(e^\epsilon - 1)}$, which is practically small. For example, in our experiments, $C$ is always smaller than $3.25 \times 10^{-4}$. Hence, the function is decreasing on the entire range of $b$. This observation will be consistent for many learning problems as soon as the size of the dataset $m$ is sufficiently large. Appropriate remarks will be made in the paper.

%When the server is trusted, the goal is for the server to output a robust statistic in a privacy-preserving manner. Hence, the server applies the privacy mechanism when computing the robust statistic. In this context, the honest workers send their gradients un-obfuscated to the server.\\
%In our setting, the server is not trusted, but honest-but-curious (refer to the threat model in Section 2). Accordingly, the noise injection scheme (for privacy against the server) is applied at the worker level, before applying any robust statistic operation at the server level. Then, the references provided by the reviewer are not applicable anymore. The honest-but-curious assumption makes the task of robust statistics more challenging, especially in non-convex settings when workers only send gradients (not actual data samples).

\subsection*{Reviewer 2}
We thank the reviewer and provide some additional feedback below.\\

\textbf{Answer to Q1:} We believe that the assumptions we make are fairly classical in optimization problems, hence we did not investigate non differentiable functions at the moment. We however believe our analysis can be adapted to non differentiable functions and this would be an interesting future direction for our work. 

\textbf{Answer to Q2:} In our paper, we only tune the hyperparameters appearing in the asymptotic error (first input to the max function in Corollary 1), which is independent of the learning rate as shown in Corollary 1. In practice, we choose a constant learning rate so that the cross-accuracy reaches the maximum level after 300 steps (in the non-private Byzantine-free setting). Our experimental findings (especially on the impact of hyperparameter tuning) are actually consistent across different learning rates.

\subsection*{Reviewer 3}
We thank the reviewer and provide more details on our contribution below.\\

\textbf{On the significance of our results:} The surprising part is the degree of improvement in the cross-accuracy when increasing the batch size, especially given the fact that doing the same has very little impact when considering the Byzantine setting (with no privacy, see Appendix E) and the private setting (with no Byzantine behavior, see "No attack" curves in Figure 2) separately.

\textbf{- Sampling procedure:} We consider empirical loss minimization where $D$ is a finite set of datapoints (not a generic distribution). The term "without replacement" refers to each honest worker sampling $b$ distinct datapoints from $D$ at each step. This sampling method is standard practice in privacy-preserving deep learning, and enables us to use existing results on DP.


\subsection*{Reviewer 4}
We thank the reviewer for their comments and provide detailed answers to their concerns below.\\

\textbf{Comments on the abstract:} \\
We only focus on the workers enforcing DP via the Gaussian mechanism, which is arguably the most standard DP mechanism in machine learning (off-the-shelf libraries implement this scheme by default, e.g.,  \href{https://github.com/tensorflow/privacy/tree/master/tensorflow_privacy}{TensorFlow Privacy}, \href{https://github.com/pytorch/opacus}{Opacus (PyTorch)}). This specification is explicitly stated in our introduction and model setting. Hence, a general analysis of the integration of DP and BR without specifying the DP mechanism, even though interesting, is out of the scope of this paper. \\

Regarding the link between VN condition and BR, please refer to our answer in below on the significance of the VN condition. \\

\textbf{Comments on the introduction:} \\
- As explained in our threat model in Section 2, our analysis considers the server to be "honest-but-curious". We only use the notion of "trusted server" in the first paragraph of the introduction to explain how distributed SGD works in the vanilla setting (i.e., without privacy and without Byzantine workers). \\

- We will provide an intuitive explanation of what Byzantine means when first introducing for completeness. \\

- We used Dwork et al (2014) to give a reference for differential privacy (DP) in general when first introducing this notion. It presents a general overview of what DP is, including a full chapter (chapter 11) on machine learning. \\

- We only cite Abadi et al. (2016)  for space limitation in the introduction. Note that we do cite Song et al. (2013) and Bassily et al. (2014) when discussing DP-SGD in Section 2.1.\\

- The main point of this informal theorem was to show how the final error is affected by the parameters of the VN condition. One does not need to fully understand the VN condition at this point but only to see that the smaller the $\eta$, the better the convergence guarantee.\\

- This sentence refers to the fact that the hyperparameters we tune in Section 4, especially the batch size $b$, have a much stronger impact on the final accuracy of the model when integrating DP and BR than when studying DP or BR separately. We give more detailed explanations on this in Sections 3 and 4 of the paper.\\

- In the experiments, the overall privacy budget is fixed but not the number of iterations as we inject more or less noise according to the batch size we consider. We did not specify this in Figure 1 as it was meant to be an illustration of our experimental results but we explain this in more detail in our experimental setting (see Section 4 and Appendix D.2).\\

\textbf{Comments on the problem setting:} \\

- By common dataset, we mean that each worker has access to the same dataset $D$; i.e., the dataset is not partitioned across workers.\\

- As we previously mentioned above, we agree that there exist other ways to provide DP besides Gaussian noise. However, this technique is the one that is most commonly implemented in machine learning libraries (Opacus and TensorFlow Privacy). When these libraries refer to DP-SGD, by default they mean Gaussian noise injection to the gradients.\\

\textbf{- Why do we consider per-step privacy?} 
We focus on per-step privacy to show that even when sacrificing privacy (running the algorithm for an infinite time), the learning error of DP-SGD with Byzantine resilience need not vanish. Moreover, it allows us to highlight the dependence of the learning error on the model hyperparameters when injecting noise of constant variance at worker-level. This observation would not have been possible to derive if the overall privacy budget was fixed a priori. It should however be noted that in our experiments, we have been careful when computing the overall privacy budget of the learning procedure as explained in Appendix D.2. \\

- Due to space limitation, we only provide a brief description of $(\alpha, f)$-Byzantine resilience. For further details, including intuition, we referred the reader to several prior works on this topic and provided several examples of such aggregation rules in Appendix B.\\

\textbf{Comments on Section 3}\\
- We never assume the identities of Byzantine and honest workers to be known by the server. Algorithm 1 is not run on one specific entity (curator/analyst), and simply delineates the instructions run by the server and the workers. The {\em for} loops for the workers simply state the actions taken by them, i.e., the term "foreach" should be read as "each".\\

- Theorem 1 is indeed derived from previous results from Dwork et al (2014) and Balle at al (2018), as we have pointed out above the theorem statement. Moreover, it remains  unclear to us how the given expression of $s \approx C^2\log(1/\delta)/\epsilon^2m^2$ guarantees the same level of privacy as ours. They may be close in the particular case where $(e^\epsilon - 1) m / b$ goes to $0$, but we do not think that this can be the case in general.\\

{\bf - Significance of VN condition} The VN condition is the only verifiable condition known in the literature to guarantee $(\alpha,f)$-BR, which has allowed researchers in the past to prove Byzantine resilience of popular GARs, e.g., {\em Krum}, {\em Phocas}, {\em MDA}, {\em Trimmed Mean} and {\em MeaMed}, {\em Bulyan}. Please refer section 3.2 of our paper and to (El-Mhamdi et al., ICLR 2021) for further details.\\

- This was indeed a typo, we meant to say that the privacy noise parameter $s$ is not zero, i.e., privacy is not meaningless. Correction will be made accordingly.\\

- $\kappa$ indeed does not appear explicitly in Theorem 2, but that does not create a mismatch of units. $\kappa$ is actually implicitly carried within the value of $\alpha$. We did not make explicit the connection between $\kappa$ and $\alpha$ for generality, because it depends on the GAR at hand. However, the value of $\alpha$ does not change our conclusions, as pointed out in Remark 1. Furthermore, note that the paper cited by the reviewer only considers convex (and strongly-convex) settings that do not apply to most neural networks which are central to our problem. We consider a general non-convex loss function, hence we do not think that it would be fair to compare our result to these previous works. \\

- Please refer to our comments above on the usefulness of per-step privacy.\\

- {\em Contextualization of our convergence result:} The result in Corollary 1 shows how the asymptotic error (i.e., regret bound when $T$ goes to infinity) depends upon the different hyperparameters of the learning algorithm (DP-SGD with BR). This analysis allows us to re-tune the hyperparameters appropriately for improving the learning accuracy of DP-SGD in the Byzantine setting. This result is especially interesting as the asymptotic error is zero (i.e., independent of hyperparameters such as $b$) in either scenarios with only DP (i.e., no Byzantine behavior) or only Byzantine resilience (i.e., no privacy guarantees). Details on this are provided below the corollary, and also in our experiments section.
